Investigating the Task Load of Investigating the Task Load in Visualization Studies

The NASA task load index (short: NASA-TLX) is a common metric to evaluate the workload of a user in a visualization study. Yet, it is rarely performed as initially intended, as the sources-of-workload evaluation is often omitted for various reasons. We conduct an online survey to investigate the task load of administering different versions of the NASA-TLX in a meta-study using the ReVISit framework. Our results show that it is not the slight increase in experiment time, but rather participants' frustration with the procedure, that contributes to the slight increase in task load when using the full version of the TLX compared to using a shortened version. However, we also show that the full version can shine a different and more faceted light on workload by adding a personal dimension to the data. We propose that a compact version of the sources-of-workload questionnaire can mitigate both time loss and frustration for study participants, while still providing the same data as the original procedure. The online study can be found and interactively explored on https://dpahr.github.io/tlxtlx/, and the source for the study, as well as the code for our analysis, can be found on https://github.com/dpahr/tlxtlx/.

==> whisker_plot.tex <==
\newcommand{\nasaWhisker}[7]{%
  \pgfmathsetmacro{\xleft}{\xpos}
  \pgfmathsetmacro{\xright}{\xpos + #7}
  \pgfmathsetmacro{\xcenter}{\xpos + #7/2}

  % Vertical line from min to max
  \draw (\xcenter,#2) -- (\xcenter,#6);

  % Whisker caps
  \draw (\xcenter,#2) -- ++(-0.15,0);
  \draw (\xcenter,#6) -- ++(-0.15,0);
  \draw (\xcenter,#2) -- ++(0.15,0);
  \draw (\xcenter,#6) -- ++(0.15,0);

  % Box from Q1 to Q3
  \draw[fill=white] (\xleft,#3) rectangle (\xright,#5);

  % Median line
  \draw[very thick] (\xleft,#4) -- (\xright,#4);

  % Label under the box
  \node[font=\bfseries] at (\xcenter, -5) {#1};

  % Advance xpos
  \pgfmathsetmacro{\xpos}{\xright + 0.2}
}

% % \nasaChart{
% \nasaChart{
%   \nasaWhisker{PD}{10}{30}{40}{60}{90}{1}
%   \nasaWhisker{MD}{20}{35}{50}{65}{80}{1.5}
%   \nasaWhisker{FR}{0}{20}{30}{40}{60}{1}  
% }{Whisker plot example}
